SoK: Yield Aggregators in DeFi

Yield farming has been an immensely popular activity for cryptocurrency holders since the explosion of Decentralized Finance (DeFi) in the summer of 2020. In this Systematization of Knowledge (SoK), we study a general framework for yield farming strategies with empirical analysis. First, we summarize the fundamentals of yield farming by focusing on the protocols and tokens used by aggregators. We then examine the sources of yield and translate those into three example yield farming strategies, followed by the simulations of yield farming performance, based on these strategies. We further compare four major yield aggregrators -- Idle, Pickle, Harvest and Yearn -- in the ecosystem, along with brief introductions of others. We systematize their strategies and revenue models, and conduct an empirical analysis with on-chain data from example vaults, to find a plausible connection between data anomalies and historical events. Finally, we discuss the benefits and risks of yield aggregators.

==> exhibits/notation.tex <==
\begin{table}
\caption{Mathematical notations for Idle Finance models}
\begin{tabularx}{8.4cm}{lX}
\toprule
Notation & Definition     \\     \midrule
$n$                 &   the number of lending protocols used          \\
$x_i$               &   the amount (in underlying) allocated in protocol $i$       \\
$nextRate(x_i)$     &   a function which returns the new APR for protocol $i$ after supplying $x_i$         \\
$nextScore(x_i)$    &   a function which returns the new Score for protocol $i$ after supplying $x_i$ amount of underlying         \\
$maxnextRate$       &   the highest rate of all implemented protocols after supplying $x_i$ amount         \\
$maxnextScore$      &   the highest score of all implemented protocols after supplying $x_i$ amount         \\
$k$                 &   a coefficient for expressing weights of score and APR         \\
$tot$               &   the total amount to rebalance  \\
\bottomrule
\end{tabularx}
\label{tab:idleFinanceNotation}
\end{table}

==> sections/appendices.tex <==
\newpage






